Nonparametric Bayesian volatility estimation for gamma-driven stochastic differential equations

We study a nonparametric Bayesian approach to estimation of the volatility function of a stochastic differential equation driven by a gamma process. The volatility function is modelled a priori as piecewise constant, and we specify a gamma prior on its values. This leads to a straightforward procedure for posterior inference via an MCMC procedure. We give theoretical performance guarantees (contraction rates for the posterior) for the Bayesian estimate in terms of the regularity of the unknown volatility function. We illustrate the method on synthetic and real data examples.

==> extensions.tex <==
\subsection{Extensions}

\subsubsection{General adjoint}
In this section we consider adjoint chains in more generality than section  \ref{adjointchain}, allowing for models without transition densities.
We assume $x_t \in \RR^{d_t}$ equipped with the Lebesgue measure as marginal reference measure.

For each $s \in \cS$ attach a Lebesgue pseudo prior density $q(x_s)$, which we incorporate by attaching an additional leaf vertex $c(s)$ at each $s \in \cS$, with $X_{c(s)}$ an arbitrary, independent random variable and $h_{c(s)}(x_s) = 1$, thus preserving the conditional distribution of $X$.
We keep using the letters $\cG$, $\cT$, $\cV_s$, etc. to denote the resulting graph, vertices, descendant leaves and set $\cC = \{c_s, s \in \cS\}$.
Set
\[
\tilde h_{c(s)}(x_s) = q(x_s),
\]
and otherwise $\tilde h_{v}(x_{\pa(v)}) = h_{v}(x_{\pa(v)})$ for $v \in \cV\setminus \cC$.
\begin{prop}
\[
\tilde h_t(x_s) =  \E \left[\prod_{v \in \cV_t}  \tilde h_v(X_{\pa(v)}) \mid X_s = x_s\right], \quad \tilde h(s, x_s) =\prod_{t \in \ch(s)}  \tilde h_t(x_s),
\]
has the telescope property \eqref{telescopetilde}.
\end{prop}

Let
\begin{equation}\label{backwardtrans}
\P^\dagger(\dd x_s \mid x_{\ch(s)}) = \mu(\dd x_s \mid  x_{\ch(s)})
\end{equation}
where
\[
\mu(\dd( x_s,  x_{\ch(s)}) ) = q(x_s) \prod_{t \in \ch(s)} \P(\dd x_t \mid x_{s}) \dd x_s.
\]
Assume that $\P^\dagger(\dd x_s \mid x_{\cV_s}) = p(x_s) \dd s$ and set $\varpi_s = \frac{ \tilde h(s, x_s)}{\tilde p(x_s)}$.




\note{I think this  can go.}}
